Investigating coronal saturation and super-saturation in fast-rotating M-dwarf stars

At fast rotation rates the coronal activity of G- and K-type stars has been observed to "saturate" and then decline again at even faster rotation rates -- a phenomenon dubbed "super-saturation". In this paper we investigate coronal activity in fast-rotating M-dwarfs using deep XMM-Newton observations of 97 low-mass stars of known rotation period in the young open cluster NGC 2547, and combine these with published X-ray surveys of low-mass field and cluster stars of known rotation period. Like G- and K-dwarfs, we find that M-dwarfs exhibit increasing coronal activity with decreasing Rossby number N_R, the ratio of period to convective turnover time, and that activity saturates at L_x/L_bol ~ 10^-3 for log N_R < -0.8. However, super-saturation is not convincingly displayed by M-dwarfs, despite the presence of many objects in our sample with log N_R < -1.8, where super-saturation is observed to occur in higher mass stars. Instead, it appears that a short rotation period is the primary predictor of super-saturation; P <=0.3d for K-dwarfs and perhaps P <=0.2d for M-dwarfs. These observations favour the "centrifugal stripping" model for super-saturation, where coronal structures are forced open or become radiatively unstable as the Keplerian co-rotation radius moves inside the X-ray emitting coronal volume.

==> latex_macros.tex <==
%
\newcommand{\rmsub}[2]{#1_{\rm #2}} 
\newcommand{\alfven}{Alfv\'en}
%
% USEFUL IN-TEXT CONTRACTIONS
%
\newcommand{\aat}{\mbox{\em AAT}}
\newcommand{\eso}{\mbox{\em ESO}}
\newcommand{\iue}{\mbox{\em IUE}}
\newcommand{\exosat}{\mbox{\em EXOSAT}}
\newcommand{\einstein}{\mbox{\em Einstein}}
\newcommand{\ginga}{\mbox{\em GINGA}}
\newcommand{\rosat}{\mbox{\em ROSAT}}
\newcommand{\caspec}{\mbox{\em CASPEC}}
\newcommand{\ucles}{\mbox{\em UCLES}}
\newcommand{\starlink}{\mbox{\em Starlink}}
\newcommand{\etal}{\mbox{\em et\ al.\ }}
\newcommand{\dex}[1]{\hbox{$\times\hbox{10}^{#1}$}}
\newcommand{\eex}[1]{\hbox{$\hbox{10}^{#1}$}}
\newcommand{\gpar}{\mbox{$g_{\parallel}$}}
\newcommand{\vsi}{\mbox{$v_e\,\sin\,i$}}
\newcommand{\vsini}{\mbox{$v_e\,\sin\,i$}}
\newcommand{\pattcit}[1]{\hbox{$^{(#1)}$}}
\newcommand{\pattcite}[1]{\hbox{$^{(#1)}$}}
%
% NAMES OF SPECTRAL LINES
%
\newcommand{\ha}{H$\alpha$}
\newcommand{\hb}{H$\beta$}
\newcommand{\hgam}{H$\gamma$}
\newcommand{\hdel}{H$\delta$}
\newcommand{\heps}{H$\epsilon$}
\newcommand{\lya}{\hbox{$\hbox{Ly}\alpha$}}
\newcommand{\naid}{\mbox{Na{\footnotesize I} {\sl D}}}
\newcommand{\caii}{Ca\,{\footnotesize II}}
\newcommand{\caiih}{Ca\,{\footnotesize II}~H}
\newcommand{\caiik}{Ca\,{\footnotesize II}~K}
\newcommand{\caiihk}{Ca\,{\footnotesize II}~H \&~K}
\newcommand{\mgii}{Mg\,{\footnotesize II}}
\newcommand{\mgiih}{\mbox{Mg{\footnotesize II} {\sl h}}}
\newcommand{\mgiik}{\mbox{Mg{\footnotesize II} {\sl k}}}
\newcommand{\mgiihk}{\mbox{Mg{\footnotesize II} {\sl h} \&\ {\sl k}}}
\newcommand{\lii}{Li\,{\footnotesize I}}
\newcommand{\fei}{Fe\,{\footnotesize I}}
\newcommand{\baii}{Ba\,{\footnotesize II}}
\newcommand{\ki}{K\,{\footnotesize I}}
\newcommand{\cai}{Ca\,{\footnotesize I}}
%
% UNITS
%
\newcommand{\ang}{\,\mbox{\AA}}
\newcommand{\Ang}{\ang}
\newcommand{\angstrom}{\ang}
\newcommand{\angstroms}{\ang}
\newcommand{\Angstrom}{\ang}
\newcommand{\Angstroms}{\ang}
\newcommand{\km}{\,km}
\newcommand{\Mpc}{\,\mbox{Mpc}}
\newcommand{\kpc}{\,\mbox{kpc}}
\newcommand{\kms}{\,km\,s$^{-1}$}
\newcommand{\ergs}{\,\mbox{$\mbox{erg}\,\mbox{s}^{-1}$}}
\newcommand{\ergsqcmsecang}{\,erg\,cm$^{-2}$\,s$^{-1}$\,\AA$^{-1}$}
\newcommand{\ergsqcm}{\,erg\,cm$^{-2}$}
\newcommand{\ergsqcmsec}{\,erg\,cm$^{-2}$\,s$^{-1}$}
\newcommand{\sqcm}{\,\mbox{$\mbox{cm}^{2}$}}
\newcommand{\cucm}{\,\mbox{$\mbox{cm}^{3}$}}
\newcommand{\persqcm}{\,\mbox{$\mbox{cm}^{-2}$}}
\newcommand{\gpersqcm}{\,\mbox{g}\persqcm}
\newcommand{\percc}{\,\mbox{$\mbox{cm}^{-3}$}}
\newcommand{\kev}{\,\mbox{keV}}
\newcommand{\kelvin}{\,K}
\newcommand{\kgmcube}{\,\mbox{$\mbox{kg}\,\mbox{m}^{-3}$}}
\newcommand{\dynsqcm}{\,\mbox{$\mbox{dyn}\,\mbox{cm}^{-2}$}}
\newcommand{\degrees}{\mbox{$^\circ$}}
\newcommand{\rstar}{\,\mbox{$\mbox{R}_*$}}
\newcommand{\mstar}{\,\mbox{$\mbox{M}_*$}}
\newcommand{\lstar}{\,\mbox{$\mbox{L}_*$}}
\newcommand{\vstar}{\,\mbox{$\mbox{V}_*$}}
\newcommand{\msun}{\,\mbox{$\mbox{M}_{\odot}$}}
\newcommand{\rsun}{\,\mbox{$\mbox{R}_{\odot}$}}
\newcommand{\lsun}{\,\mbox{$\mbox{L}_{\odot}$}}
\newcommand{\lx}{\,\mbox{$L_{\rm x}$}}
%
% REFERENCES
%
\newcommand{\reference}[5]{\noindent #1, #2. {\sl #3\/}, {\bf #4,} \,\mbox{#5}} 
\newcommand{\refnum}[4]{\noindent #1, #2. {\sl #3\/}, {\bf #4}}
\newcommand{\refbook}[3]{\noindent #1, #2. {\sl #3\/}}
\newcommand{\refpress}[3]{\noindent #1, #2. {\sl #3\/}, in press}
\newcommand{\refsub}[3]{\noindent #1, #2. {\sl #3\/}, submitted}
\newcommand{\refprep}[2]{\noindent #1, #2. In preparation}
%
% JOURNAL ABBREVIATIONS
%
\newcommand{\aanda}  {Astr.\ Astro\-phys.\nolinebreak\ }
\newcommand{\aasupp} {Astr.\ Astro\-phys.\nolinebreak\ Suppl.\nolinebreak\ }
\newcommand{\aj}     {Astron.\nolinebreak\ J.\nolinebreak\ }
\newcommand{\annrev} {Ann.\ Rev.\ Astr.\ Astro\-phys.\nolinebreak\ }
\newcommand{\acta}   {Acta Astron.\nolinebreak\ }
\newcommand{\apj}    {Astro\-phys.\nolinebreak\ J.\nolinebreak\ }
\newcommand{\apjs}   {Astro\-phys.\nolinebreak\ J.\ Suppl.\nolinebreak\ }
\newcommand{\apjsupp}{\apjs}
\newcommand{\aplett} {Astro\-phys.\nolinebreak\ Lett.\nolinebreak\ }
\newcommand{\gafd}   {Geo\-phys.~Astro\-phys.\ Fluid Dyn.\nolinebreak\ }
\newcommand{\ibvs}   {Inf.\ Bull.\ var.\ Stars\nolinebreak\ }
\newcommand{\jgr}    {J.\ Geo\-phys.~Res.\nolinebreak\ } 
\newcommand{\jpp}    {J.\ Plasma Phys.\nolinebreak\ }
\newcommand{\mn}     {Mon.\ Not.\ R.\ astr.\nolinebreak\ Soc.\nolinebreak\ }
\newcommand{\pf}     {Phys.\nolinebreak\ Fluids\nolinebreak\ }
\newcommand{\pasp}   {Publ.\ astr.\ Soc.\ Pacif.\nolinebreak\ }
\newcommand{\sovast} {Soviet astr.\nolinebreak\ }
\newcommand{\procasa}{Proc.\ Astr.\ Soc.\ Australia\nolinebreak\ }
\newcommand{\solp}   {Solar Phys.\nolinebreak\ }
\newcommand\mnras{MNRAS}
\newcommand\aap  {A\&A}
\newcommand\aaps  {A\&AS}

%
% MATH MACROS
%
\newcommand{\der}[1]{{\rm d}#1}
\newcommand{\deriv}[2]{\frac{{\rm d}#1}
                       {{\rm d}#2}} 
\newcommand{\sderiv}[2]{\frac{{\rm d}^2#1}\over
                       {{\rm d}#2^2}} 
\newcommand{\pderiv}[2]{\frac{\partial#1}
                       {\partial#2}} 
\newcommand{\spderiv}[2]{\frac{\partial^2#1}
                        {\partial#2^2}} 
\newcommand{\half}{\mbox{$\frac{1}{2}$}}
\newcommand{\twiddles}{\mbox{$\sim $}}
\newcommand{\varomega}{\varpi}
\newcommand{\twid}{\mbox{$\sim $}}
\newcommand{\bvec}[1]{\mbox{\boldmath ${#1}$}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bd}{\begin{displaymath}}
\newcommand{\ed}{\end{displaymath}}
\newcommand{\del}{{\bf \nabla}}












